Efficient and Effective Tree-based and Neural Learning to Rank

This monograph takes a step towards promoting the study of efficiency in the era of neural information retrieval by offering a comprehensive survey of the literature on efficiency and effectiveness in ranking, and to a limited extent, retrieval. This monograph was inspired by the parallels that exist between the challenges in neural network-based ranking solutions and their predecessors, decision forest-based learning to rank models, as well as the connections between the solutions the literature to date has to offer. We believe that by understanding the fundamentals underpinning these algorithmic and data structure solutions for containing the contentious relationship between efficiency and effectiveness, one can better identify future directions and more efficiently determine the merits of ideas. We also present what we believe to be important research directions in the forefront of efficiency and effectiveness in retrieval and ranking.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> makefile <==
### Makefile for LaTeX under Mac OS X
### Author: Franco Maria Nardini (francomaria.nardini@isti.cnr.it)
# pdflatex, textmate, and skim are needed to run properly all the commands here.

# Some assumptions:
# ./img: is the directory containing images
# ./style: is the directory containing the .cls and .sty

# NAME OF THE MAIN FILE (WITHOUT .tex)
BASEFILENAME=paper

# NAME OF THE CAMERA READY FILE (WITHOUT .pdf)
DESTFILENAME=

# NAME OF THE TEXTMATE PROJECT FILE
PROJECTFILENAME=

pdf:
	@pdflatex ${BASEFILENAME}.tex
	@biber ${BASEFILENAME}
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex
	@open -a skim ${BASEFILENAME}.pdf &

pdf-cameraready:
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex
	@mv ${BASEFILENAME}.pdf ${DESTFILENAME}.pdf
	@open -a skim ${DESTFILENAME}.pdf

pdf-coverletter:
	@pdflatex letter.tex
	bibtex letter
	@pdflatex letter.tex
	@pdflatex letter.tex
	@rm letter.aux letter.log

images:
	@for filename in `ls ./img/*.eps`; do epstopdf $$filename; done;

count:
	@pdftotext ${BASEFILENAME}.pdf WORDS
	@wc --words WORDS
	@rm -f WORDS

clean:
	@rm -f ./img/*~ *~ *spl .*.lb *loa *aux *dvi *maf *mtc *mtc0 *log *fls *lof *lot *out ${BASEFILENAME}.pdf *bbl *blg *idx *toc *txt *fdb_latexmk *synctex*

edit:
	@open -a textmate ${PROJECTFILENAME}.tmproj &

chkrefs:
	@bibtex ${BASEFILENAME}

tgz:
	@tar -czf $(PWD)\ `date +%Y%m%d%H%M`.tar.gz *tex *tmproj *bib ./img/* ./style/*

commit:
	@svn update
	@svn commit -m "`date +%Y%m%d%H%M` - FM"

update:
	@svn update

